Quanta in sound, the sound of quanta: a voice-informed quantum theoretical perspective on sound

Humans have a privileged, embodied way to explore the world of sounds, through vocal imitation. The Quantum Vocal Theory of Sounds (QVTS) starts from the assumption that any sound can be expressed and described as the evolution of a superposition of vocal states, i.e., phonation, turbulence, and supraglottal myoelastic vibrations. The postulates of quantum mechanics, with the notions of observable, measurement, and time evolution of state, provide a model that can be used for sound processing, in both directions of analysis and synthesis. QVTS can give a quantum-theoretic explanation to some auditory streaming phenomena, eventually leading to practical solutions of relevant sound-processing problems, or it can be creatively exploited to manipulate superpositions of sonic elements. Perhaps more importantly, QVTS may be a fertile ground to host a dialogue between physicists, computer scientists, musicians, and sound designers, possibly giving us unheard manifestations of human creativity.

==> QVTS_arxiv/references.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
%\biblstarthook{
% References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} If the citation in the text is numbered, the reference list should be arranged in ascending order. If the citation in the text is author/year, the reference list should be \textit{sorted} alphabetically and if there are several works by the same author, the following order should be used:
%\begin{enumerate}
%\item all works by the author alone, ordered chronologically by year of publication
%\item all works by the author with a coauthor, ordered alphabetically by coauthor
%\item all works by the author with several coauthors, ordered chronologically by year of publication.
%\end{enumerate}
%The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
%\begin{itemize}
%\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
%\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
%\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
%\item Examples of the basic Springer Nature style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
%\end{itemize}
%}

\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 
%\bibitem{science-contrib} Broy, M.: Software engineering --- from auxiliary to key technologies. In: Broy, M., Dener, E. (eds.) Software Pioneers, pp. 10-13. Springer, Heidelberg (2002)
%
% Online Document
%\bibitem{science-online} Dod, J.: Effective substances. In: The Dictionary of Substances and Their Effects. Royal Society of Chemistry (1999) Available via DIALOG. \\
%\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
%\bibitem{science-mono} Geddes, K.O., Czapor, S.R., Labahn, G.: Algorithms for Computer Algebra. Kluwer, Boston (1992) 
%
% Journal article
%\bibitem{science-journal} Hamburger, C.: Quasimonotonicity, regularity and duality for nonlinear systems of partial differential equations. Ann. Mat. Pura. Appl. \textbf{169}, 321--354 (1995)



%
% Journal article by DOI
%\bibitem{science-DOI} Slifka, M.K., Whitton, J.L.: Clinical implications of dysregulated cytokine production. J. Mol. Med. (2000) doi: 10.1007/s001090000086 
%
%\bigskip

\bibitem{asaka2020}
Asaka, R., Sakai, K., and Yahagi, R.: Quantum circuit for the fast Fourier transform. Quantum Information Processing, {\bf 19}, 277 (2020)

\bibitem{aspect1982}
Aspect, A., and Dalibard, J., and Roger, G.: Experimental test of Bell's inequalities using time-varying analyzers. Physical review letters {\bf 49} (25), 1804 (1982)


\bibitem{blutnerGraben20}
Blutner, R., beim Graben, P.: Gauge models of musical forces. J. of Math. and Music, (2020)  doi: 10.1080/17459737.2020.1716404

\bibitem{bell}
Bell, J. S.: On the Einstein Podolsky Rosen Paradox. Physics Physique Fizika. \emph{1} (3): 195--200 (1964) \url{doi:10.1103/PhysicsPhysiqueFizika.1.195}

\bibitem{bigand2000divided}
Bigand, E., McAdams, S., and For{\^e}t, S.: Divided attention in music. International Journal of Psychology {\bf 35} 6, 270--278 (2000)

%\bibitem{bilbao2004}
%Bilbao, S.: Wave and scattering methods for numerical simulation. John Wiley \& Sons (2004)


\bibitem{bogdanov2013essentia}
Bogdanov, D., Wack, N., G\'{o}mez Guti\'{e}rrez, E., Gulati, S., Herrera Boyer, P., Mayor, O., Roma Trepat, G., Salamon, J., Zapata Gonz\'{a}lez, J. R., and Serra, X.: Essentia: An audio analysis library for music information retrieval. In: Proc. of the 14th Conference of the International Society for Music Information Retrieval (ISMIR), 493--498, Curitiba, Brazil, 2013

\bibitem{bonada2011spectral}
Bonada, J., Serra, X., Amatriain, X., and Loscos, A.: Spectral processing, in Z\"olzer, U. (Editor): DAFX: Digital Audio Effects, 393--445, John Wiley \& Sons, Ltd (2011)

\bibitem{bregman1994auditory}
Bregman, A. S.: Auditory scene analysis: The perceptual organization of sound. MIT Press: Cambridge, MA (1994)

\bibitem{brown2020}
Brown, A. R.: Playing Pool with $|\psi\rangle$: from Bouncing Billiards to Quantum Search. Quantum { \emph 4}, 357, Verein zur F{\"o}rderung des Open Access Publizierens in den Quantenwissenschaften (2020) 





\bibitem{byrne}
Byrne, \'{A}., Rinzel, J., Rankin, J.: Auditory streaming and bistability paradigm extended to a dynamic environment.  Hearing Research \emph{383}, 107807 (2019)
 
\bibitem{cadiz}
C\'{a}diz, R., and Ramos, J.: Sound Synthesis of a Gaussian Quantum Particle in an Infinite Square Well. Computer Music Journal \emph{38} (4), 53--67 (2014)

\bibitem{cariolaro2015quantum}
Cariolaro, G.: Quantum communications. Cham: Springer (2015)

\bibitem{ciocca1987}
Ciocca, V., and Bregman, A. S.: Perceived continuity of gliding and steady-state tones through interrupting noise. Perception \& Psychophysics {\bf 42} 5, 476--484, Springer (1987)

\bibitem{synthesizer_AM}
Costa Hamido, O., and Cirillo, G. A., and Giusto, E.: Quantum synth: a quantum-computing-based synthesizer. In: Proceedings of the 15th International Conference on Audio Mostly, 265--268 (2020)

\bibitem{dallaChiara}
Dalla Chiara, M. L., Giuntini, R., Leporini, R., Negri, E., Sergioli, G.: Quantum information, cognition, and music. Frontiers in Psych. \textbf{6}, 1583 (2015)

\bibitem{daniloff1973}
Daniloff, R.G., and Hammarberg, R.E.: On defining coarticulation. Journal of Phonetics {\bf 1} (3), 239--248 (1973) http://www.sciencedirect.com/science/article/pii/S0095447019313889

% issn = "0095-4470"

\bibitem{delleMonache2018}
Delle Monache, S., Rocchesso, R., Bevilacqua, F., Lemaitre, G., Baldan, S., Cera, A.: Embodied sound design. International Journal of Human-Computer Studies {\bf 118}, 47--59 (2018)

\bibitem{epr}
Einstein, A., Podolsky, B., and Rosen, N.: Can quantum-mechanical description of physical reality be considered complete? Physical Review \emph{41}, 777 (1935) Retrieved online from \url{http://www.drchinese.com/David/EPR.pdf}

\bibitem{feynman}
Feynman, R.: The Character of Physical Law. Cambridge (MA), MIT Press (1995)

\bibitem{friberg2018}
Friberg, A., Lindeberg, T.,  Hellwagner, M., Helgason, P.,  Salom$\tilde{\mbox{a}}$o, G. L., Elowsson, A., Lemaitre,G., and Ternstr\"{o}m, S.: Prediction of three articulatory categories in vocal sound imitations using models for auditory receptive fields. The Journal of the Acoustical Society of America {\bf 144} (3), 1467--1483 (2018)


\bibitem{gabor}
Gabor, D.: Acoustical quanta and the theory of hearing. Nature \emph{159}, 4044, 591 (1947)

\bibitem{gaver}
Gaver, W. W.: What in the world do we hear? An ecological approach o auditory event perception. Ecological Psychology. {\bf 5} (4), 285 (1993)

\bibitem{GHIRARDI1999}
Ghirardi, G.: Quantum superpositions and definite perceptions: envisaging new feasible experimental tests. Physics Letters A  {\bf 262} (1), 1--14 (1999)

\bibitem{irino}
Irino, T., and Patterson, R. D.: A time-domain, level-dependent auditory filter: The gammachirp. The Journal of the Acoustical Society of America, {\bf 101} (1), 412--419 (1997)

\bibitem{helmholtz}
von Helmholtz, H.: Die Lehre von den Tonempfindungen als physiologische Grundlagef\"{u}rdie Theorie
der Musik. Braunschweig, F. Vieweg und sohn (1870)

\bibitem{jot1997}
Jot, J.-M.: Efficient models for reverberation and distance rendering in computer music and virtual audio reality. In: Proceedings: International Computer Music Conference 1997, Thessaloniki, Hellas, 25-30 September 1997, 236--243, The International Computer Music Association (1997)

\bibitem{juett}
Juett, J. C.: Pauline Oliveros and Quantum Sound. Liminalities: A Journal of Performance Studies {\bf 6} (2), 1--10 (2010) http://liminalities.net/6-2/oliveros.pdf

\bibitem{koenig}
Koenig, D. M., and Delwin, D. F.: Spectral Analysis of Musical Sounds with Emphasis on the Piano. (New York, Oxford University Press, 2015)

\hide{\bibitem{sonify}
Kontogeorgakopoulos, A., and Burgarth, D.: Sonification of controlled quantum dynamics. Proceedings of the 2014 International Computer Music Conference, 1432--1436 (2014)
}

%\bibitem{kubovy2}
%Kubovy, M., and Van Valkenburg, D.: Auditory and Visual Objects. Cognition {\bf 80} (1--2), 97--126 (2001)

\bibitem{cella}
Kulpa, J., Campion, E., and Cella, C.: QuBits, a System for Interactive Sonic Virtual Reality. Proceedings of ICMC 2020,Santiago, Chile (2020). Retrieved from\url{http://www.carminecella.com/research/2020_ICMC_QuBits.pdf}

\bibitem{kulpa}
Kulpa, J.: QuBits, an Interactive Virtual Reality Project and Compositional Space for Sound and Image. Advisor: E. Campion. PhD dissertation, Berkeley, California (2019). Retrieved online from \url{https://escholarship.org/uc/item/5tq9x2hb}

\hide{\bibitem{rocchesso_lemaitre}
Lemaitre, G., Rocchesso, D.: On the effectiveness of vocal imitations and verbal descriptions of sounds. The Journal of the Acoustical Society of America \emph{135} (2), 862 (2014) Retrieved online from \url{https://iris.unipa.it/retrieve/handle/10447/370549/745030/1.4861245.pdf}}


\bibitem{receptive_fields}
Lindeberg, T., and Friberg, A.: Idealized Computational Models for Auditory Receptive Fields. PLoS ONE {\bf 10} (3), e0119032. https://doi.org/10.1371/journal.pone.0119032
	
\bibitem{GestART}
Mannone, M., Favali, F., Di Donato, B., Turchet, L. Quantum GestART: identifying and applying correlations between mathematics, art, and perceptual organization. J. Math. Music (2020) doi: 10.1080/17459737.2020.1726691

\bibitem{gest_sim}
Mannone, M.: Introduction to gestural Similarity. An application of category theory to the orchestra. J. Math Music {\bf 12} (2), 63--87 (2018) 

\bibitem{mannone_compagno}
Mannone, M., and Compagno, G.: Characterization of the degree of Musical non-Markovianity. ArXiV (2014) Retrieved online from \url{https://arxiv.org/abs/1306.0229}

\bibitem{marinetti}
Marinetti, F. T.: Zang tumb tumb. Milano, Edizioni futuriste di poesia (1914) Retrieved online from \url{http://parliamoitaliano.altervista.org/zang-tumb-tumb/}

\bibitem{miranda2021a}
Miranda, E. R.: Quantum Computer: Hello, Music! In: E. Miranda (Ed.), Handbook of Artificial Intelligence for Music: Foundations, Advanced Approaches, and Developments for Creativity. Springer Nature (2021)

\bibitem{miranda2021b}
Miranda, E. R.: Creative Quantum Computing: Inverse FFT Sound Synthesis, Adaptive Sequencing and Musical Composition. In: A. Adamatzky (Ed.), Alternative Computing, World Scientific (2021)

\bibitem{newman2004}
Newman, F.: MouthSounds: How to Whistle, Pop, Boing, and Honk... for All Occasions and Then Some. Workman Publishing (2004)

\bibitem{NielsenChuang2010}
Nielsen, M. A., and Chuang, I. L.: Quantum Computation and Quantum Information. Cambridge University Press (2010) 
	
	
\bibitem{oliveros1999}
Oliveros, P.: Quantum listening: From practice to theory (to practise practice). In: K. Siu Tong and C. Sin-wai, Culture and Humanity in the New Millennium: The Future of Human Values. The Chinese University Press, 27--44 (2002)


\bibitem{palazzeschi}
Palazzeschi, A.: La fontana malata, from Poemi. Firenze, Cesare Blanc (1909) Retrieved online from \url{https://www.pensieriparole.it/poesie/poesie-d-autore/poesia-38384}

\bibitem{pohlmann1995}
Pohlmann, K. C.: Principles of Digital Audio, USA, McGraw-Hill, Inc., 3rd edition (1995)

% isbn = {0070504687}

\bibitem{pulkki2011spatial}
Pulkki, V., Lokki, T., and Rocchesso, D.: Spatial effects. DAFX: Digital Audio Effects, 139--183, Wiley (2011)

\bibitem{roads2001}
Roads, C.: Microsound. Cambridge, MA: MIT Press (2001)

\bibitem{rocchesso2016}
Rocchesso, D., Mauro, D., and Drioli, C.: Organizing a sonic space through vocal imitations. J. Audio Eng. Soc. {\bf 64} 7/8, 474--483 (2016) http://www.aes.org/e-lib/browse.cfm?elib=18333

\bibitem{rocchesso1995}
Rocchesso, D.: The Ball within the Box: A Sound-Processing Metaphor. Computer Music journal {\bf 4} (19), 47--57, The MIT Press (1995) http://www.jstor.org/stable/3680990

 % ISSN = {01489267, 15315169},

\bibitem{rocchesso1997}
Rocchesso, D.: Maximally diffusive yet efficient feedback delay networks for artificial reverberation. IEEE Signal Processing Letters, {\bf 4} (9), 252--255 (1997) 10.1109/97.623041

\bibitem{QVTS}
Rocchesso, D., Mannone, M.: A quantum vocal theory of sound. Quantum Inf. Proc. \textbf{19}, 292 (2020) doi: 10.1007/s11128-020-02772-9

\bibitem{mimic2016}
Rocchesso, D., Mauro, D. A., and Delle Monache, S.: MiMic: The Microphone as a Pencil. Proceedings of the TEI '16: Tenth International Conference on Tangible, Embedded, and Embodied Interaction, in Eindhoven, Netherlands. Association for Computing Machinery, 357--364, TEI '16, New York, NY, USA (2016) https://doi.org/10.1145/2839462.2839467
% doi = {10.1145/2839462.2839467},



% the following reference has nothing to do with skat-vg (which came five years later
\hide{\bibitem{skat-vg}
SKAT-VG project: https://cordis.europa.eu/project/id/618067/it}
%Rocchesso, D., and Serafin, S.: Sonic Interaction Design (Special issue). International Journal of Human-Computer Studies \emph{67} (11), 905--994 (2009)

\bibitem{rovelli}
Rovelli, C.: Helgoland. Penguin Books(2021)

\bibitem{SalamonGomez2012}
Salamon, J., and Gomez, E.: Melody Extraction From Polyphonic Music Signals Using Pitch Contour Characteristics. IEEE Transactions on Audio, Speech, and Language Processing {\bf 20} 6, 1759--1770 (2012)

\bibitem{schlecht2017}
Schlecht, S. J., and Habets, E. A. P.: On Lossless Feedback Delay Networks. IEEE Transactions on Signal Processing, {\bf 65} (6), 1554--1564 (2017) 10.1109/TSP.2016.2637323

\bibitem{schlecht2020}
Schlecht, S. J.: FDNTB: The feedback delay network toolbox. In: Proceedings of the 23rd International Conference on Digital Audio Effects DAFx-20 (2020)

\bibitem{shamma}
Shamma S.: Spectro-Temporal Receptive Fields. In: Jaeger D., Jung R. (eds) Encyclopedia of Computational Neuroscience. Springer, New York, NY (2013) \url{https://doi.org/10.1007/978-1-4614-7320-6_437-1}

%\bibitem{shannon}
%Shannon, C. E.: Communication in the Presence of Noise. Proceedings of the IRE \emph{37} (1), 10 (1949) Retrieved online from \url{http://shilov-sss.ru/wp-content/uploads/2018/05/Shannon-C.-Communication-in-the-presence-of-noise-PIRE-37-I-194910.pdf}

%\bibitem{skat-vg}
%Sonic Interaction Design
% SKAT-VG: Sketching Audio Technologies using Vocalizations and Gestures. (2016) \url{http://www.iuav.it/Ricerca1/LA-RICERCA/PROGETTI-D/PROGETTI-D/RICERCHE-I/VII-PROGRA/SKAT-VG/SKATVG_2.pdf}

\bibitem{spence_multi}
Spence, C., Senkowski, D., and R\"{o}der, B.: Crossmodal processing. Exp Brain Res {\bf 198} (107), 107--111 (2009). Retrieved online from \url{https://link.springer.com/article/10.1007/s00221-009-1973-4}

\bibitem{spence}
Spence, C.: Crossmodal correspondences: A tutorial review. Attention, Perception, \& Psychophysics {\bf 73}, 971--995 (2011) Retrieved online from \url{https://doi.org/10.3758/s13414-010-0073-7}

\bibitem{verma}
Verma, T. S., Levine, S. N., and Meng, T. H.: Transient Modeling Synthesis: a flexible analysis/synthesis tool for transient signals. Proceedings of the International Computer Music Conference, 48--51 (1997)

\bibitem{vochlea}
Vochlea microphone. Retrieved online from \url{https://vochlea.com/}


\bibitem{vicario1963}
Vicario, G. B.: La ``dislocazione temporale'' nella percezione di successioni di stimoli discreti (The ``time displacement'' in the perception of sequences of discrete stimuli). Rivista di Psicologia, {\bf 57} 1, 17--87 (1963)


\bibitem{vicario1960effetto}
Vicario, G: L’effetto tunnel acustico (The acoustic tunnel effect). Rivista di Psicologia {\bf 54}, 41--52 (1960)

\hide{\bibitem{wavelet}
Wavelet. Wikipedia (2020) Retrieved online from \url{https://en.wikipedia.org/wiki/Wavelet}}

\bibitem{Weimer2010}
Weimer, H.: Listen to Quantum Computer Music. \url{http://www.quantenblog.net/physics/quantum-computer-music}, Accessed: 2021-01-02 (2010)

\bibitem{yearsley}
Yearsley, J.M., and Busemeyer,  J.R.: Foundations of Probability Theory in Psychology and Beyond (special issue). Journal of Mathematical Psychology {\bf 74}, 99 (2016)

\bibitem{youssry}
Youssry, A., El-Rafei, A., and Elramly, S.: A quantum mechanics-based framework for image processing and its application to image segmentation. Quantum Information Processing {\bf 14} (10), 3613--3638 (2015)

% Use the following (APS) syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Online Document
%\bibitem{phys-online} J. Dod, in \textit{The Dictionary of Substances and Their Effects}, Royal Society of Chemistry. (Available via DIALOG, 1999), 
%\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
%\bibitem{phys-mono} H. Ibach, H. L\"uth, \textit{Solid-State Physics}, 2nd edn. (Springer, New York, 1996), pp. 45-56 
%
% Journal article
%\bibitem{phys-journal} S. Preuss, A. Demchuk Jr., M. Stuke, Appl. Phys. A \textbf{61}
%
% Journal article by DOI
%\bibitem{phys-DOI} M.K. Slifka, J.L. Whitton, J. Mol. Med., doi: 10.1007/s001090000086
%
% Contribution 
%\bibitem{phys-contrib} S.E. Smith, in \textit{Neuromuscular Junction}, ed. by E. Zaimis. Handbook of Experimental Pharmacology, vol 42 (Springer, Heidelberg, 1976), p. 593
%
%\bigskip
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Psychology, Social Sciences"
%
%
% Monograph
%\bibitem{psysoc-mono} Calfee, R.~C., \& Valencia, R.~R. (1991). \textit{APA guide to preparing manuscripts for journal publication.} Washington, DC: American Psychological Association.
%
% Online Document
%\bibitem{psysoc-online} Dod, J. (1999). Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
%\url{http://www.rsc.org/dose/Effective substances.} Cited 15 Jan 1999.
%
% Journal article
%\bibitem{psysoc-journal} Harris, M., Karper, E., Stacks, G., Hoffman, D., DeNiro, R., Cruz, P., et al. (2001). Writing labs and the Hollywood connection. \textit{J Film} Writing, 44(3), 213--245.
%
% Contribution 
%\bibitem{psysoc-contrib} O'Neil, J.~M., \& Egan, J. (1992). Men's and women's gender role journeys: Metaphor for healing, transition, and transformation. In B.~R. Wainrig (Ed.), \textit{Gender issues across the life cycle} (pp. 107--123). New York: Springer.
%
% Journal article by DOI
%\bibitem{psysoc-DOI}Kreger, M., Brindis, C.D., Manuel, D.M., Sassoubre, L. (2007). Lessons learned in systems change initiatives: benchmarks and indicators. \textit{American Journal of Community Psychology}, doi: 10.1007/s10464-007-9108-14.
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Humanities, Linguistics, Philosophy"
%
%\bigskip
%
% Journal article
%\bibitem{humlinphil-journal} Alber John, Daniel C. O'Connell, and Sabine Kowal. 2002. Personal perspective in TV interviews. \textit{Pragmatics} 12:257--271
%
% Contribution 
%\bibitem{humlinphil-contrib} Cameron, Deborah. 1997. Theoretical debates in feminist linguistics: Questions of sex and gender. In \textit{Gender and discourse}, ed. Ruth Wodak, 99--119. London: Sage Publications.
%
% Monograph
%\bibitem{humlinphil-mono} Cameron, Deborah. 1985. \textit{Feminism and linguistic theory.} New York: St. Martin's Press.
%
% Online Document
%\bibitem{humlinphil-online} Dod, Jake. 1999. Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
%http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999
%
% Journal article by DOI
%\bibitem{humlinphil-DOI} Suleiman, Camelia, Daniel C. O'Connell, and Sabine Kowal. 2002. `If you and I, if we, in this later day, lose that sacred fire...': Perspective in political interviews. \textit{Journal of Psycholinguistic Research}. doi: 10.1023/A:1015592129296.
%
%
%
%\bigskip
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Computer Science, Economics, Engineering, Geosciences, Life Sciences"
%
%
% Contribution 
%\bibitem{basic-contrib} Brown B, Aaron M (2001) The politics of nature. In: Smith J (ed) The rise of modern genomics, 3rd edn. Wiley, New York 
%
% Online Document
%\bibitem{basic-online} Dod J (1999) Effective Substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
%\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Journal article by DOI
%\bibitem{basic-DOI} Slifka MK, Whitton JL (2000) Clinical implications of dysregulated cytokine production. J Mol Med, doi: 10.1007/s001090000086
%
% Journal article
%\bibitem{basic-journal} Smith J, Jones M Jr, Houghton L et al (1999) Future of health insurance. N Engl J Med 965:325--329
%
% Monograph
%\bibitem{basic-mono} South J, Blass B (2001) The future of modern genomics. Blackwell, London 
%
\end{thebibliography}

